Explaining Giant Apparent $\mathrm{p}K_\mathrm{A}$ Shifts in Weak Polyelectrolyte Brushes

Recent experiments on weak polyelectrolyte brushes found marked shifts in the effective p$K_\mathrm{A}$ that are linear in the logarithm of the salt concentration. Comparing explicit-particle simulations with mean-field calculations we show that for high grafting densities the salt concentration effect can be explained using the ideal Donnan theory, but for low grafting densities the full shift is due to a combination of the Donnan effect and the polyelectrolyte effect. The latter originates from electrostatic correlations which are neglected in the Donnan picture and which are only approximately included in the mean-field theory. Moreover, we demonstrate that the magnitude of the polyelectrolyte effect is almost invariant with respect to salt concentration but depends on the grafting density of the brush. This invariance is due to a complex cancellation of multiple effects. Based on our results, we show how the experimentally determined p$K_\mathrm{A}$ shifts may be used to infer the grafting density of brushes, a parameter that is difficult to measure directly.

==> arxiv_submission_2/authors-title.tex <==
\title{Explaining Giant Apparent $\pKa$ Shifts in Weak Polyelectrolyte Brushes}

\author{David Beyer}
\affiliation{Institute for Computational Physics, University of Stuttgart, D-70569 Stuttgart, Germany}

\author{Peter Košovan}
\email{peter.kosovan@natur.cuni.cz}
\affiliation{Department of Physical and Macromolecular Chemistry, Charles University, Prague, Czechia}


\author{Christian Holm}%
\email{holm@icp.uni-stuttgart.de}
\affiliation{Institute for Computational Physics, University of Stuttgart, D-70569 Stuttgart, Germany}




==> arxiv_submission_2/authors-title_esi.tex <==
\title{Supplementary Material: Explaining Giant Apparent $\pKa$ Shifts in Weak Polyelectrolyte Brushes}

\author{David Beyer}
\affiliation{Institute for Computational Physics, University of Stuttgart, D-70569 Stuttgart, Germany}

\author{Peter Košovan}
\email{peter.kosovan@natur.cuni.cz}
\affiliation{Department of Physical and Macromolecular Chemistry, Charles University, Prague, Czechia}


\author{Christian Holm}%
\email{holm@icp.uni-stuttgart.de}
\affiliation{Institute for Computational Physics, University of Stuttgart, D-70569 Stuttgart, Germany}


==> arxiv_submission_2/definitions.tex <==
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\etal}{\emph{et al}}
\newcommand{\kb}{k_\mathrm{B}}
\newcommand{\lb}{\lambda_\mathrm{B}}
\newcommand{\ld}{\lambda_\mathrm{D}}
\newcommand{\lp}{l_\mathrm{p}}
\newcommand{\lB}{l_\mathrm{Bjerrum}}
\newcommand{\kT}{k_\mathrm{B}T}
\newcommand{\Rend}[0]{R_\mathrm{e}}
\newcommand{\Rout}[0]{R_\mathrm{out}}
\newcommand{\Rstar}{R_{\mathrm{star}}}
\newcommand{\Rbox}{R_{\mathrm{box}}}
\newcommand{\Rmax}{R_{\mathrm{max}}}
\newcommand{\Ro}{R_\mathrm{0}}
\newcommand{\Fpo}{F^\mathrm{po}}
\newcommand{\avg}[1]{\left<{#1}\right>}
\newcommand{\lan}{{\cal{L}}}
\newcommand{\ilan}{{\cal{L}}^{-1}}
\newcommand{\Deltadon}{\Delta^\mathrm{Don}}
\newcommand{\muref}{\mu^{\ominus}}
\newcommand{\muid}{\mu^\mathrm{id}}
\newcommand{\muex}{\mu^\mathrm{ex}}
\newcommand{\musalt}{\mu_\mathrm{s}}
\newcommand{\brush}{^{\mathrm{brush}}}
\newcommand{\cs}{c_\mathrm{salt}}
\newcommand{\cmon}{c_\mathrm{mon}}
\newcommand{\zmon}{z_\mathrm{mon}}
\newcommand{\ccat}{c_{\mathrm{cat}}}
\newcommand{\can}{c_{\mathrm{an}}}
\newcommand{\Pel}{P_\mathrm{el}}
\newcommand{\Pstr}{P_\mathrm{str}}
\newcommand{\Posm}{P_\mathrm{osm}}
\newcommand{\Pbox}{P_\mathrm{box}}
\newcommand{\Pext}{P_\mathrm{ext}}
\newcommand{\Req}{R_\mathrm{eq}}
\newcommand{\Veq}{V_\mathrm{eq}}
\newcommand{\Qeq}{Q_\mathrm{eq}}
\newcommand{\QV}{Q_{\mathrm{V}}}
\newcommand{\QR}{Q_{\mathrm{\Rend}}}
\newcommand{\Vbox}{V_\mathrm{box}}
\newcommand{\Vchain}{V_\mathrm{chain}}
\newcommand{\Pin}[0]{P_\mathrm{in}}

\newcommand{\Aall}{\mathrm{A}}
\newcommand{\HA}{\mathrm{HA}}
\newcommand{\Aminus}{\mathrm{A}^{-}}
\newcommand{\Clminus}{\mathrm{Cl}^{-}}
\newcommand{\Naplus}{\mathrm{Na}^{+}}
\newcommand{\Hplus}{\mathrm{H}^{+}}
\newcommand{\OHminus}{\mathrm{OH}^{-}}
\newcommand{\cHplus}{c_{\Hplus}}
\newcommand{\cref}{c^{\ominus}}
\newcommand{\muna}{\mu_\mathrm{Na}}
\newcommand{\mucl}{\mu_\mathrm{Cl}}
\newcommand{\muh}{\mu_\mathrm{H}}
\newcommand{\muoh}{\mu_\mathrm{OH}}
\newcommand{\cH}{\ensuremath{c_{\Hplus{}}}}
\newcommand{\cOH}{\ensuremath{c_{\OHminus{}}}}
\newcommand{\cNa}{\ensuremath{c_{\Naplus{}}}}
\newcommand{\cCl}{\ensuremath{c_{\Clminus{}}}}
\newcommand{\cA}{\ensuremath{c_{\ce{A-}}}}
\newcommand{\cHres}{\ensuremath{\cH\res{}}}
\newcommand{\cOHres}{\ensuremath{\cOH\res{}}}
\newcommand{\cNares}{\ensuremath{\cNa\res{}}}
\newcommand{\cClres}{\ensuremath{\cCl\res{}}}


\newcommand{\Vo}{V_\mathrm{0}}
\newcommand{\Vd}{V_\mathrm{d}}

\newcommand{\Van}{\overline{V}_\mathrm{an}}
\newcommand{\Vcat}{\overline{V}_\mathrm{cat}}
\newcommand{\Vs}{\overline{V}_\mathrm{s}}
\newcommand{\Vw}{\overline{V}_\mathrm{w}}
\newcommand{\Vm}{\overline{V}_\mathrm{m}}

\newcommand{\gel}{^{\mathrm{gel}}}
\newcommand{\res}{^{\mathrm{res}}}

\newcommand{\der}{\mathrm{d}} % for todal derivative
\newcommand{\Nav}{N_{\mathrm{A}}}
\newcommand{\nubar}{\bar{\nu}}


\newcommand{\Kw}{K_{\mathrm{w}}}
\newcommand{\pKw}{\mathrm{p}K_{\mathrm{w}}}
\newcommand{\pK}{\mathrm{p}K}
\newcommand{\pKa}{\mathrm{p}K_{\mathrm{A}}}
\newcommand{\pKeff}{\pKa^{\mathrm{eff}}}
\newcommand{\app}{^{\mathrm{app}}}
\newcommand{\pH}{\mathrm{pH}}
\newcommand{\pHsys}{\pH\gel}
\newcommand{\pHres}{\pH\res}
\newcommand{\Ires}{I\res}

\newcommand{\pI}{\mathrm{p}\idp}
\newcommand{\pOH}{\mathrm{pOH}}

\newcommand{\es}{\textsc{ESPResSo}\xspace}
\newcommand{\ES}{\es}

\newcommand{\idp}{\ensuremath{I}}
\newcommand{\idpAB}{\ensuremath{\idp_{\sA{}\sB{}}}}
\newcommand{\idpAD}{\ensuremath{\idp_{\sA{}\sD{}}}}
\newcommand{\idpCB}{\ensuremath{\idp_{\sC{}\sB{}}}}
\newcommand{\idpCD}{\ensuremath{\idp_{\sC{}\sD{}}}}
\newcommand{\idps}{\ensuremath{\mathcal{I}^2}}
\newcommand{\idpsAB}{\ensuremath{\idps_{\sA{}\sB{}}}}
\newcommand{\idpsAD}{\ensuremath{\idps_{\sA{}\sD{}}}}
\newcommand{\idpsCB}{\ensuremath{\idps_{\sC{}\sB{}}}}
\newcommand{\idpsCD}{\ensuremath{\idps_{\sC{}\sD{}}}}

\newcommand*{\KNaCl}{K_{\mathrm{Na+Cl}}}
\newcommand*{\KHCl}{K_{\mathrm{H+Cl}}}
\newcommand*{\KNaOH}{K_{\mathrm{Na+OH}}}
\newcommand*{\KHNa}{K_{\mathrm{Na-H}}}
\newcommand*{\KOHCl}{K_{\mathrm{Cl-OH}}}
\newcommand*{\KHOH}{K_{\mathrm{H+OH}}}

% Figure and equation references
\newcommand{\reffig}[1]{Fig.~\ref{#1}}
\newcommand{\refsec}[1]{Section~\ref{#1}}
\newcommand{\refeq}[1]{Eq.~\ref{#1}}

\newcommand{\epsilonr}{\epsilon_\mathrm{r}}

% red strikeout
\usepackage[normalem]{ulem} % enables command \sout for strikeout
\newcommand{\soutr}[1]{\sout{\textcolor{red}{#1}}}
\newcommand{\soutb}[1]{\sout{\textcolor{blue}{#1}}}
% shorthand for my blue
\newcommand{\myblue}[1]{\textcolor{blue}{#1}}
\newcommand{\myred}[1]{\textcolor{red}{#1}}
% uncomment the line below to produce pdf in the final form, without the strikeouts and colours
\renewcommand{\soutr}[1]{\relax}
\renewcommand{\soutb}[1]{\relax} \renewcommand{\myblue}[1]{#1} \renewcommand{\myred}[1]{#1}

